Renormalization Group Guided Tensor Network Structure Search

Tensor network structure search (TN-SS) aims to automatically discover optimal network topologies and rank configurations for efficient tensor decomposition in high-dimensional data representation. Despite recent advances, existing TN-SS methods face significant limitations in computational tractability, structure adaptivity, and optimization robustness across diverse tensor characteristics. They struggle with three key challenges: single-scale optimization missing multi-scale structures, discrete search spaces hindering smooth structure evolution, and separated structure-parameter optimization causing computational inefficiency. We propose RGTN (Renormalization Group guided Tensor Network search), a physics-inspired framework transforming TN-SS via multi-scale renormalization group flows. Unlike fixed-scale discrete search methods, RGTN uses dynamic scale-transformation for continuous structure evolution across resolutions. Its core innovation includes learnable edge gates for optimization-stage topology modification and intelligent proposals based on physical quantities like node tension measuring local stress and edge information flow quantifying connectivity importance. Starting from low-complexity coarse scales and refining to finer ones, RGTN finds compact structures while escaping local minima via scale-induced perturbations. Extensive experiments on light field data, high-order synthetic tensors, and video completion tasks show RGTN achieves state-of-the-art compression ratios and runs 4-600$\times$ faster than existing methods, validating the effectiveness of our physics-inspired approach.

==> 6CheckList.tex <==
\clearpage


\section*{Reproduction Checklist}
\subsection*{Methodology Description}
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced. \hfill \textit{yes}
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results. \hfill \textit{yes}
    \item Provides well marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper. \hfill \textit{yes}
\end{itemize}

\subsection*{Theoretical Contributions}
\begin{itemize}
    \item Does this paper make theoretical contributions? \hfill \textit{yes} \\
    \textit{If yes, please complete the list below.}
    \begin{itemize}
        \item All assumptions and restrictions are stated clearly and formally. \hfill \textit{yes}
        \item All novel claims are stated formally (e.g., in theorem statements). \hfill \textit{yes}
        \item Proofs of all novel claims are included. \hfill \textit{partial}
        \item Proof sketches or intuitions are given for complex and/or novel results. \hfill \textit{yes}
        \item Appropriate citations to theoretical tools used are given. \hfill \textit{yes}
        \item All theoretical claims are demonstrated empirically to hold. \hfill \textit{yes}
        \item All experimental code used to eliminate or disprove claims is included. \hfill \textit{yes}
    \end{itemize}
\end{itemize}

\subsection*{Datasets}
\begin{itemize}
    \item Does this paper rely on one or more datasets? \hfill \textit{yes} \\
    \textit{If yes, please complete the list below.}
    \begin{itemize}
        \item A motivation is given for why the experiments are conducted on the selected datasets. \hfill \textit{yes}
        \item All novel datasets introduced in this paper are included in a data appendix. \hfill \textit{yes}
        \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \hfill \textit{yes}
        \item All datasets drawn from the existing literature are accompanied by appropriate citations. \hfill \textit{yes}
        \item All datasets drawn from the existing literature are publicly available. \hfill \textit{yes}
        \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. \hfill \textit{NA}
    \end{itemize}
\end{itemize}

\subsection*{Computational Experiments}
\begin{itemize}
    \item Does this paper include computational experiments? \hfill \textit{yes} \\
    \textit{If yes, please complete the list below.}
    \begin{itemize}
        \item This paper states the number and range of values tried per (hyper-)parameter during development, along with the criterion used for selecting the final parameter setting. \hfill \textit{NA}
        \item Any code required for pre-processing data is included in the appendix. \hfill \textit{yes}
        \item All source code required for conducting and analyzing the experiments is included in a code appendix. \hfill \textit{yes}
        \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \hfill \textit{yes}
        \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from. \hfill \textit{yes}
        \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. \hfill \textit{yes}
        \item This paper specifies the computing infrastructure used for running experiments (hardware and software). \hfill \textit{yes}
        \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. \hfill \textit{yes}
        \item This paper states the number of algorithm runs used to compute each reported result. \hfill \textit{yes}
        \item Analysis of experiments goes beyond single-dimensional summaries of performance to include measures of variation, confidence, or other distributional information. \hfill \textit{yes}
        \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). \hfill \textit{partial}
        \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. \hfill \textit{yes}
    \end{itemize}
\end{itemize}
